Effective Monitoring of Online Decision-Making Algorithms in Digital Intervention Implementation

Online AI decision-making algorithms are increasingly used by digital interventions to dynamically personalize treatment to individuals. These algorithms determine, in real-time, the delivery of treatment based on accruing data. The objective of this paper is to provide guidelines for enabling effective monitoring of online decision-making algorithms with the goal of (1) safeguarding individuals and (2) ensuring data quality. We elucidate guidelines and discuss our experience in monitoring online decision-making algorithms in two digital intervention clinical trials (Oralytics and MiWaves). Our guidelines include (1) developing fallback methods, pre-specified procedures executed when an issue occurs, and (2) identifying potential issues categorizing them by severity (red, yellow, and green). Across both trials, the monitoring systems detected real-time issues such as out-of-memory issues, database timeout, and failed communication with an external source. Fallback methods prevented participants from not receiving any treatment during the trial and also prevented the use of incorrect data in statistical analyses. These trials provide case studies for how health scientists can build monitoring systems for their digital intervention. Without these algorithm monitoring systems, critical issues would have gone undetected and unresolved. Instead, these monitoring systems safeguarded participants and ensured the quality of the resulting data for updating the intervention and facilitating scientific discovery. These monitoring guidelines and findings give digital intervention teams the confidence to include online decision-making algorithms in digital interventions.

==> 00_abstract/abstract.tex <==
\begin{abstract}
Autonomous decision-making algorithms are increasingly used in digital intervention  trials to dynamically personalize treatments to participants. These algorithms determine, in real-time, the delivery of treatment based on accruing participant data during the conduct of the trial.  While there exists standard practices for monitoring other trial components (e.g., participant monitoring, data monitoring, etc.), the inclusion of an online decision-making algorithm requires additional monitoring.  Successful deployment of the algorithm requires: (1) safeguarding participants and (2) ensuring data excellence for post-trial analyses. In this paper, we elucidate  guidelines and discuss our experience in  monitoring online decision-making algorithms  in two digital intervention clinical trials. These trials provide case studies for how health scientists can build  monitoring systems for their digital intervention  trial.

% Autonomous decision-making algorithms are increasingly used in clinical trials to dynamically personalize treatments to participants. There exists standard practices for monitoring other components (e.g., participant monitoring, data monitoring, etc.). However, the introduction of an online decision-making algorithm means additional monitoring is required. This is because such algorithms adjust treatment based on incoming data and participant responses as the trial is running. Successful deployment involves interactions with many complex systems make it challenging to ensure: (1) quality participant experience and (2) data excellence for post-trial analyses. In this paper, we apply the framework originally proposed in \citet{trella2024monitoring} to offer guidelines for monitoring online decision-making algorithms monitoring systems in clinical trials with 2 case studies. By actuating the ideas from the framework, we show how other scientific teams can build a simiar monitoring system for their clinical trial.
% We make their ideas more concrete and applicable and showcase how one can build a similar monitoring system for a new clinical trial.
\end{abstract}



==> related_work/main.tex <==
\section{Related Work}
\label{related_work}

\alt{TODO: we need to re do this section to related to work in the clinical trials literature that already exists.}

Meeting with Stefan:
Current monitoring in clinical trials without an adaptive algorithm (e.g. fixed protocol like AB testing or ABAB testing)

Any clinical trial has a safety component, what are potential events? How are you going to track, monitor, and how to deal with adverse events

* standard non digital: manual patient feedback: enter symptoms, or called by the study nurse, clinical staff check ins. Emergency they have a phone number they can call.
* digital but not adaptive: direct feedback from participants (e.g., the app is not working) participants will email or call staff. They want to eventually implement some logging through the app or something. Logging helps with when the participant reports an issue with the app. There’s no passive sensing on whether the participant did the treatment (e.g., did they actually go for a walk). Since the treatment is set, monitoring is not on the treatment protocol but on all the digital components supporting sending the treatment (i.e., app)
* digital and adaptive (us): 

To help research teams best prepare for RL algorithm deployment in the challenging healthcare setting, we introduce \textit{algorithm fidelity}: the responsibility of the online RL algorithm in (1) safeguarding participants and (2) preserving the scientific utility of the data in clinical trials. These concepts build upon quality control and data quality, which are two well-defined criteria for ML deployment. Quality control, used widely throughout engineering, encompasses a comprehensive set of standards or predefined set of requirements that a product must meet before launching. Data quality involves best practices of handling or reporting the data used to train models. Here, we extend quality control and data quality to concerns involving online RL algorithms in clinical trials.
% Our algorithm fidelity framework extends quality control standards that considerations that involve protecting participants and data quality to practices that ensure the scientific utility of the data.
% Quality control and data quality are two key considerations discussed in existing literature on best practices for ML model deployment. 
% These concepts are consistent with existing work in RL algorithm design where one must consider how the algorithm 1) runs stably and automatically without the need for constant human monitoring (consistent functionality and reliability) and 2) involves proper documentation and reproducibility of results \citep{a15080255}. 
Often times, other system components (see Appendix~\ref{app_other_forms_fidelity}) are also responsible for ensuring quality control and data quality. However, algorithm fidelity specifically refers to areas that are directly controlled or caused by the RL algorithm. For example, monitoring for app crashes and failing to collect app analytics falls under the purview of the clinician dashboard. However, detecting errors in saving state values used to select actions would come under monitoring of algorithm fidelity.

\subsection{Related Work}
\label{related_work}
We build on quality control and data quality discussed in the existing literature on best-practice frameworks for deploying ML models in general and discuss how they can be adapted to online RL algorithms in clinical trials. 
% Quality control and data quality are significantly studied in the literature for general ML systems and some specific to health. 
Many of the ML frameworks for ensuring quality control or data quality are in the offline or in batch settings where the algorithm is trained on previous batch data and the model is fixed before deployment.
In these settings, quality control standards could include achieving baseline prediction accuracy \citep{oala2021machine}, handling distribution shifts and reporting levels of confidence \citep{challen2019artificial}, explainability, fairness, and reproducibility \citep{oala2020ml4h, loftus2022ideal}, or preparing for accidents and unintended risks \citep{amodei2016concrete}.
%that a new version of the model is stable and meets validation criteria. 
Data quality could include ensuring that models trained on the data can accurately represent and predict for their task \citep{sambasivan2021everyone}, or forming a checklist of what to report about AI algorithms in clinical trials such as which version of the algorithm was used, how input data was acquired, and how the sample size was determined \citep{liu2020reporting}.

%1) protecting participants and 2) ensuring that the data collected during the trial can be used for after-study analyses (continual learning, off-policy evaluation, causal inference, etc.).
\subsection{Quality Control}
\label{quality_control}
The online nature and inherent properties of RL algorithms require additional aspects of quality control. Unlike prediction models, validating the quality of RL algorithms goes beyond straightforward performance metrics like prediction accuracy. Also, online algorithms autonomously update using incoming data from participants in the trial. Previous work covers monitoring the deployment of between-trial algorithm updates with a fixed policy \citep{oala2020ml4h}, but online settings require identifying and addressing issues in real-time of a policy that is frequently updated throughout the trial. Furthermore, validation in the online setting is more complicated than in the offline setting. In the offline setting, training can involve a human-in-the-loop \citep{wu2022survey} for performing hyperparameter search, checking for convergence, or performing clinical evaluations \citep{oala2020ml4h}. An online algorithm, however, can only be validated once the trial has completed (e.g., via off-policy analyses, one can evaluate whether an action  was effective in certain states for a participant).

Considering our clinical trial setting, we also extend quality control to include standards that involve participant experience and safety. In any clinical trial, participant protection from harm and adverse experiences is the most important consideration. Although there is a list of ethical guidelines that the clinical research team must follow (i.e., overseen by Institutional Review Boards \citep{grady2015institutional}) 
%\sam{might cite  https://www.ncbi.nlm.nih.gov/pmc/articles/PMC4631034/} 
and guidelines that must be followed to  register the trial (i.e., at clinicaltrials.gov) \footnote{The framework considers participant protection responsible by the RL algorithm as opposed to general participant protection guidelines in the trial. Note that ethics are priority consideration prior to algorithmic development. For example, in trials where the algorithm actions may have negative side effects (e.g., administering a drug), the action space is restricted by the current state of the participant. 
%\kwz{For digital experiments more generally, this seems related to ensuring a basic level of user experience (to prevent user disengagement/exit)}
%and an additional level of monitoring is required.
% data safety monitoring board Cite DSMB peeps. to register the trial, all actions of the algorithm need to be approved to even register the trial and get IRB approval. Therefore the RL algorithm, for example in a setting that is unsafe or can cause the participant harm such as interrupting the participant while the participant is driving.
}, 
unintended harm can occur via the inappropriate choice of actions by the RL algorithm. For example, the algorithm could deliver too many interventions that take the participant away from normative activities and may lead to burden, habituation, and subsequent dropout. On the other hand, the algorithm could deliver too few interventions or none at all, thus diminishing the intended health benefits of the intervention actions. Furthermore, the algorithm could reduce the functionality of the participant's smartphone by depleting the battery or taking up a large amount of storage space.   
%\alt{By the time we even register the trial, participant protection involves preventing burden.}

%Patient experience involves how a patient feels about receiving care. %perception of care
%Patient experience is a key contributor to patient trust in the healthcare system and clinical effectiveness in improving health outcomes \cite{greenfield1985expanding, stewart1995effective}. 
% found this article: https://uk.sodexo.com/inspired-thinking/insights/what-is-patient-experience.html#:~:text=Better%20patient%20experiences%20are%20associated,between%20cleanliness%20and%20infection%20prevention. but they don't cite their sources.
% In our digital intervention setting, the RL algorithm directly affects the quality of patient experience through basic software functionality of the algorithm and assigning treatment.

% After-study Analyses: reproducibility and scientific usability of data (primary analyses, causal inference, off-policy evaluation, comparing two algorithms)

\subsection{Data Quality}
\label{sec_scientific_utility}
Achieving data quality for online RL algorithms is also not straightforward. RL algorithms use and store additional types of data as compared to ML algorithms, such as the action-selection probability $\pi_{i, t}$ for every participant $i$ at decision-time $t$. 
 % Comparing online algorithms to offline algorithms also requires additional effort in maintaining quality control. 
Online algorithms also require extra considerations for data reporting and reproducibility. Unlike offline settings where previous work suggests stating the version of the model used \citep{liu2020reporting}, frequent updates of the RL algorithm in the online setting means needing to index and save each policy update, the data that was used in each update, and code versions and software packages if a code change needed to be made during the trial.
%we have many frequent updates where one needs to track the software version, the policy, and the data associated with forming that policy. 

We also extend data quality in our setting to focus on preserving the scientific utility of data for post-trial analyses. Post-trial analyses refers to the broad range of analyses conducted after the trial is completed. These kinds of analyses can (1) improve the design of the intervention for future iterations; (2) inform policy and decisions for rolling out the intervention more broadly; and (3) support the development and refinement of health behavior theories. We now highlight some important analyses of interest. At a minimum, the clinical trial must collect data to perform a primary analysis \citep{furberg2012approaches,qian2022microrandomized}, a statistical analysis that addresses the foremost scientific question of the trial. For example, the primary analysis for Oralytics concerns the causal excursion
% average \sam{  This is not the average effect but rather a causal excursion effect.  Then reference tianchen's and audrey's papers for a definition of the causal excursion effect: Qian, T., Walton, A., Collins, L.M., Klasnja, P., Lanza, S., Nahum-Shani, I., Rabbi, M., Russell, M., Walton, M.A., Yoo, H. and Murphy, S.A. The Micro-Randomized Trial for Developing Digital Interventions: Experimental Design and Data Analysis Considerations (2022), Psychological Methods, 27(5), 874–894. PMC9276848 https://doi.org/10.1037/ ;      For you, Anna: the primary analysis is always about inference concerning some kind of causal effect. }
effect \citep{boruvka2018assessing} of sending versus not sending a prompt on the participant's proximal oral self-care behaviors. Secondary analysis may focus on investigating whether the benefits of sending (versus not sending) a prompt vary by the participant's baseline characteristics (e.g., age and gender), as well as their current state (e.g., recent brushing quality or app engagement). Additional analyses such as off-policy evaluation \citep{thomas2016data, levine2020offline}, other types of causal inference \citep{ hadad2021confidence}, 
%algorithm comparison \alt{ANNA TODO: Anna can't find any good cites on this. Maybe should we delete?}, 
and continual learning \citep{parisi2019continual, khetarpal2022towards} %loo2020generalized
assess the benefit of using such an algorithm and improve the design of future versions of the RL algorithm. Furthermore, sharing and publishing high-quality trial data helps the broader scientific community design their own algorithm for future trials.

% Ensuring the scientific utility of the data means the data is usable to stakeholders for running primary analyses, causal inference, off-policy evaluation, algorithm comparison, and continual learning. \alt{tell them what primary analysis is. find a cite for almost everything.} 

==> related_works.tex <==
\subsection{Literature on AI in Clinical Trials}

Two big things they talk about: 1) quality control (validtion, monitoring, reproducibility), and 2) data excellence (reporting, auditing, replicability of study). It's much more challenging for us because of the online nature of our algorithm.

Key Contributions Of Our Paper:
\begin{itemize}
    \item Detecting unique issues of an online algorithm in real-time (e.g., patient dosage beyond networking or system-level issues).
    \item Online property of algorithm produces the need for real-time monitoring (most people consider offline batch training).
    \item Most people talk about monitoring the deployment of the algorithm with a fixed policy. But not necessarily the \textit{fidelity} algorithm. Unintended negative consequences can affect patient experience during the study because of the online nature of the algorithm.
\end{itemize}

\paragraph{Types of papers in literature}
\begin{itemize}
    \item AI Quality Control: Considerations when designing, deploying, and monitoring AI models for health care and other high-stakes settings. Auditing.
    \alt{We are different because quality control is much harder when running and online algorithm. The online property of the algorithm produces the need for real-time monitoring (most people consider offline batch training). Autonomous updating.}
    \item Data reporting,  reproducibility, and data excellence in clinical trials \kwz{We are different because need to be able to reproduce the algorithm itself which has randomness and is updating. What does data excellence mean in the online decision making setting in clinical trials.}
\end{itemize}

\paragraph{Summary of papers:}
\begin{itemize}
    \item \bo{Artificial intelligence, bias and clinical safety.} Talk about training and deployment of AI models for healthcare (rather than algorithms that learn online). They discuss issues like distributional shift, explainability, unsafe failure modes. Short term, medium term, long term considerations \kwz{Focus is on potential unintended consequences (bias, failure modes, distribution shift) of deploying AI. Esp for supervised learning.}
    \alt{We contribute a framework for monitoring an \textit{online} algorithm: ``ML systems that are very frequently updated, and particularly those that continuously learn". This contributes trust towards clinical safety.}
    \item \bo{Reporting guidelines for clinical trial reports for interventions involving artificial intelligence: the CONSORT-AI extension.} Checklist for what to report about AI algorithms in clinical trials (versus clinical trials not using AI algorithms). For example, which version of algorithm used, how input data acquired, data quality, etc. \kwz{checklists for enhancing reproducibility and scientific validity} \alt{They mention reporting which version of the algorithm was used. We go into more detail and mention this doesn't just include the software version but also the policy that was used. Do they also mention the importance of reproducing the algorithm? Just knowing the version sometimes is not enough.}
    \item \bo{Artificial intelligence in dental research: Checklist for authors, reviewers, readers.} Study design, Data, Sampling, Data Protection, Missing data Data Processing, Reference Test, Sample Size, Model, Model parameters Training, Justify the best- performing model, Evaluation, Uncertainty Explainability Results \kwz{checklists for enhancing reproducibility and scientific validity}
    \item \bo{Artificial intelligence to enhance clinical value across the spectrum of cardiovascular healthcare.} Following a clear research hypothesis, an AI-based workflow begins with data selec- tion and pre-processing prior to analysis, with the type of data (structured, semi-structured, or unstructured) determining what type of pre-pro- cessing steps and machine-learning algorithms are required. Algorithmic and data validation should be performed to ensure the robustness of the chosen methodology, followed by an objective evaluation of performance. Seven case studies are provided to highlight the wide variety of data modalities and clinical questions that can benefit from modern AI techniques, with a focus on applying them to cardiovascular disease management. \kwz{AI workflow from data to training to deployment. A lot of focus is on supervised or unsupervised learning methods, rather than online algorithms.}
    \item \bo{Concrete Problems in AI Safety.} he problem of accidents in machine learning systems, defined as unintended and harmful behavior that may emerge from poor design of real-world AI systems. We present a list of five practical research problems related to accident risk, categorized according to whether the problem originates from having the wrong objective function (“avoiding side effects” and “avoiding reward hacking”), an objective function that is too expensive to evaluate frequently (“scalable supervision”), or undesirable behavior during the learning process (“safe exploration” and “distributional shift”). \kwz{Awareness of potential unintended consequences of AI deployment.}
    \item \bo{“Everyone wants to do the model work, not the data work”: Data Cascades in High-Stakes AI.} Data Cascades: compounding events causing negative, downstream efects from data issues, result- ing in technical debt4 over time. In our study, data cascades were widely prevalent: 92\% of AI practitioners reported experiencing one or more, and 45.3\% reported two or more cascades in a given project. Data cascades often resulted from applying conventional AI practices that undervalued data quality.
    \alt{highlights how poor data quality or undervaluing data in high-stakes domain have out-sized effects on living beings} \alt{Authors also mentioned that high-stakes AI often combines two or more disciplines. Challenge: greater collaboration. One example this comes up in Oralytics is we have to communicate to and have a contract with all systems on the data they provide and are saving. For example, main controller didn't know they needed to save the actual prompt of messages that are scheduled.} \alt{``Production iw the process of deploying systems `live', with a need to keep systems running smoothly and scaling efficiently."} \alt{Our paper: obtaining data excellence in the online RL clinical trial setting.}
    \item \bo{Ideal algorithms in healthcare: Explainable, dynamic, precise, autonomous, fair, and reproducible.} explainable (convey the relative importance of features in determining outputs), dynamic (capture temporal changes in physiologic signals and clinical events), precise (use high-resolution, multimodal data and aptly complex architecture), autonomous (learn with minimal supervision and execute without human input), fair (evaluate and mitigate implicit bias and social inequity), and reproducible (validated externally and prospectively and shared with academic communities). \kwz{importance of data quality and curation in real world deployments}
    \item \bo{ML4H Auditing: From Paper to Practice.} However, their transla- tion into medical practice is often ham- pered by a lack of careful evaluation in different settings. Efforts have started worldwide to establish guidelines for evaluating machine learning for health (ML4H) tools, highlighting the neces- sity to evaluate models for bias, inter- pretability, robustness, and possible fail- ure modes. However, testing and adopt- ing these guidelines in practice remains an open challenge. In this work, we tar- get the paper-to-practice gap by apply- ing an ML4H audit framework proposed by the ITU/WHO Focus Group on Arti- ficial Intelligence for Health (FG-AI4H) to three use cases: diagnostic prediction of diabetic retinopathy, diagnostic pre- diction of Alzheimer’s disease, and cyto- morphologic classification for leukemia diagnostics. The assessment comprises dimensions such as bias, interpretability, and robustness. \kwz{ideal qualities of algorithms for healthcare}
    \item \bo{Machine Learning for Health: Algorithm Auditing and Quality Control.} 
    the deployment of machine learning for health (ML4H) tools into real-world applications has been slow because existing approval pro- cesses [6] may not account for the particular failure modes and risks that accompany (ML) technology. In order to overcome this hurdle, we envision a frame- work of algorithm auditing and quality control that provides a path towards the effective and reliable application of ML systems in healthcare. \alt{Their updates are manual, between-trial updates.
    We are dealing with autonomous, real-time, within-trial updates.}
    \alt{Deployment and Monitoring look different for us. Even how you validate also looks different for us.}
    \begin{itemize}
        \item The typical ML product life cycle goes through stages of planning, development, validation and, potentially, deployment under appropriate monitoring (see Fig. 1B). Feedback loops between stages, for example from product validation back to development, are commonplace.
        \item An audit entails a detailed assessment of an ML4H tool at one or more of the ML life cycle steps. It can be carried out to anticipate, monitor, or retrospectively review operations of the tool. The audit output should consist of a comprehensive standardized report that can be used by different stakeholders to efficiently communicate the tool’s strengths and limitations
        \item \bo{Facet 1: technical validation} application of data and ML model quality assessment methods to detect possible failure modes in the model’s behavior. These include model-oriented metrics, such as predictive performance, robustness, interpretability, disparity or uncertainty, but also data oriented metrics related to sample size determination, sparseness, bias, distribution mismatch and label quality
        \item \bo{Facet 2: Clinical Evaluation} o analyse whether there is sufficient clinical evidence to confirm compliance with relevant essential requirements for safety and performance when using the device according to the manufacturer’s instructions for use
        \item \bo{Facet 3: Regulatory Assessment}
        \item \bo{Life cycle: plan, develop, validate, deploy and monitor}
    \end{itemize}
    \kwz{Focus a lot on supervised learning / rather than RL alg considerations. }
    \item \bo{Randomized Clinical Trials of Machine Learning Interventions in Health Care.} systematically examine the design, reporting standards, risk of bias, and inclusivity of RCTs for medical machine learning interventions.  Common reasons for nonadherence were not assessing poor-quality or unavailable input data (38 trials [93\%]), not analyzing performance errors (38 [93\%]), and not including a statement regarding code or algorithm availability (37 [90\%]). Overall risk of bias was high in 7 trials (17\%). Of 11 trials (27\%) that reported race and ethnicity data, the median proportion of participants from underrepresented minority groups was 21\% (range, 0\%-51\%). \kwz{Reasons behind not following clnical trial reporting guidelines/checklists. Reasons included not analyzing performance errors, not assessing input data, not including statement on algorithm availability / code.} 
    
    \item \bo{Guidelines for clinical trial protocols for interventions involving artificial intelligence: the SPIRIT-AI extension.}  The SPIRIT-AI extension includes 15 new items that were considered sufficiently important for clinical trial protocols of AI interventions. These new items should be routinely reported in addition to the core SPIRIT 2013 items. SPIRIT-AI recom- mends that investigators provide clear descriptions of the AI intervention, including instructions and skills required for use, the setting in which the AI intervention will be integrated, considerations for the handling of input and output data, the human–AI interaction and analysis of error cases. SPIRIT-AI will help promote transparency and completeness for clinical trial protocols for AI interventions. Its use will assist editors and peer reviewers, as well as the general readership, to understand, interpret and critically appraise the design and risk of bias for a planned clinical trial. \kwz{Similar to CONSORT-AI paper.}
\end{itemize}
